Flee the Flaw: Annotating the Underlying Logic of Fallacious Arguments Through Templates and Slot-filling

Prior research in computational argumentation has mainly focused on scoring the quality of arguments, with less attention on explicating logical errors. In this work, we introduce four sets of explainable templates for common informal logical fallacies designed to explicate a fallacy's implicit logic. Using our templates, we conduct an annotation study on top of 400 fallacious arguments taken from LOGIC dataset and achieve a high agreement score (Krippendorf's alpha of 0.54) and reasonable coverage (0.83). Finally, we conduct an experiment for detecting the structure of fallacies and discover that state-of-the-art language models struggle with detecting fallacy templates (0.47 accuracy). To facilitate research on fallacies, we make our dataset and guidelines publicly available.

==> recycle_bin.tex <==

%%% RECYCLE BIN
%%%Moved to a separate file to make searching in main file easier.

% \item Our experiments show that fallacy logic structure identification poses a significant challenge for state-of-the-art language models like GPT-3.5 and GPT-4 (\S\ref{sec:experiments}).
%\end{itemize}



% In the realm of argument education, elucidating implicit assumptions within arguments is pivotal for providing constructive feedback. This study delves into computational argumentation with the aim of enhancing educational tools through the analysis of argumentation, implicit messaging, and feedback provision. Distinguishing between valid and invalid arguments—fallacies being the latter due to flawed reasoning—this research focuses on structuring the analysis of fallacies for educational purposes. It endeavours to explicitly define premises and conclusions in informal arguments, detect underlying assumptions (between-line message), and highlight fallacious reasoning, thereby contributing significantly to the education domain.





% % An argument consists of two fundamental elements: premises and a conclusion, together creating a cohesive series of sentences. Arguments can be classified as either valid or invalid according to the concept of validity. The concept of validity pertains to the quality of the argument, particularly emphasizing the connection between the premises and the conclusion. Conversely, invalid arguments are characterized by flawed reasoning, often referred to as fallacies. 


% This research specifically concentrates on informal fallacies, where the invalidity arises from the content of the argument rather than its structure~\cite{van2021informal}. Suppose the argument in Figure~\ref{fig:overview}: 
% % \begin{itemize}
% %     \item \textit{I took an NLP class, an advanced course in Stanford. I suggest not taking further advanced courses because they will hurt your GPA.}
% % \end{itemize}
% This argument is classified as \textit{faulty generalization} fallacy because it generalizes into not taking further advanced courses based on taking an NLP class.
% Exercising such fallacious arguments leads to manipulation and the obscuration of truth, making it necessary to detect and explain why these arguments are fallacious~\cite {Hinton2020EvaluatingArgument}.

% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=\linewidth]{figure/figure_1_new.pdf}
% %     \caption{An overview of our fallacious argument instantiation task. Inspired by~\cite{reisert2018feasible}, we focus on Argument from Consequences~\cite{walton2008argumentation} schemes to create a list of new fallacy templates composed of slot-fillers and argumentative components for our new, challenging task.}
% %     \label{fig:overview}
% % \end{figure}


% % Previous research has concentrated on establishing benchmark datasets to examine fallacious arguments. Notable contributions in this field include the ElecDeb60To16-fallacy dataset by Goffredo et al. (2022), Argotario by Habernal et al. (2017), and the LOGIC dataset by Jin et al. (2022). Particularly, the LOGIC dataset, sourced from various student quiz websites, serves an educational aim by assisting students in understanding fallacies. Its easy accessibility and straightforwardness make it a valuable resource in educational environments focused on learning about fallacies. However, these datasets have a notable limitation: they lack comprehensive explanations for the fallacies they feature. This gap hinders the development of critical thinking skills, especially in educational settings.

% % Furthermore, the use of argument templates, commonly applied for mapping annotation schemes, has not been extensively explored in the context of fallacious arguments. Various argumentation corpora, such as~\cite{reed2006preliminary}, which annotated the Araucaria corpus using~\cite{walton2008argumentation} argumentation scheme, and~\cite{lawrence2016argument}, which developed a framework for instantiating argumentation schemes through natural language templates, have not calculated inter-annotator agreement. Additionally, \newcite{reisert2018feasible} employed templates inspired by argument from consequence to annotate the arg-microtexts corpus~\cite{peldszus2015annotated}, highlighting the underlying reasoning in arguments. Despite these advancements, the application of templates in the fallacious domain remains unexplored.

% % Template-based approaches have proven effective in explicating implicit knowledge within arguments, offering ease of control and consistency in annotation~\cite{singh-etal-2022-irac,mim-etal-2022-lpattack,naito-etal-2022-typic}. Since implicit knowledge often contributes to vagueness and assumption-making in arguments, making it explicit through templates enhances understanding because explicit knowledge is straightforward. This is particularly beneficial in identifying fallacies, which can be challenging due to their implicit components~\cite{10.1093/acprof:oso/9780198713241.003.0010}.


% Previous research in the field has primarily focused on developing benchmark datasets for the analysis of fallacious arguments, with significant contributions such as the ElecDeb60To16-fallacy dataset by \newcite{goffredo2022fallacious}. However, the exploration of argument templates for annotating fallacies has been limited. Despite various efforts in argumentation corpora to employ templates for clearer reasoning representation, the specific application of these templates to fallacious arguments has not been extensively investigated. Template-based approaches, advocated by recent studies, offer a method for making implicit knowledge in arguments explicit, thereby facilitating the identification of fallacies by clarifying their underlying assumptions~\cite{singh-etal-2022-irac,mim-etal-2022-lpattack,naito-etal-2022-typic}. This approach underscores the potential of templates in enhancing the understanding and consistency of annotations within the domain of fallacy analysis.

% To address the existing gap in research, we introduce innovative templates designed for identifying structures of fallacies across four prevalent types found in daily discourse. These templates convert implicit semantic meanings into explicit structures. We focus on two dimensions: firstly, developing new detection schemes for explainable fallacy identification with the help of expert annotators; and secondly, assessing the effectiveness of these templates against leading tools, including prompt engineering techniques with few-shot learning on GPT 4 model. Our findings indicate that these templates significantly enhance large language models' ability to detect and understand the nuanced meanings embedded in fallacious arguments.



% %   An overview of our task is shown in Figure~\ref{fig:overview}. Inspired by Argumentation Schemes~\cite{walton2008argumentation} and argument templates~\cite{reisert2018feasible}, we create an inventory of fallacy templates consisting of slot-fillers and argumentative components based on the most common argumentation scheme type (i.e., Argument from Consequences).
% % As many fallacy types exist in the wild~\cite{tindale2007fallacies}, we select 4 informal logical fallacy (i.e., fallacy of defective induction~\cite{sourati2023robust}) as a start for exploring creating a fallacy template. This research compiles 400 instances, across four fallacy types (i.e., \textit{faulty generalization}, \textit{false dilemma}, \textit{fallacy of credibility}, and \textit{false causality}). We assessed the Inter-Annotator Agreement (IAA) using three different statistical measures: Cohen's Kappa, Gwet's AC1, and Krippendorff's alpha, to ensure reliability and consistency in the annotations.

% % The research involved two rounds of annotation: one for developing the annotation guidelines with the Development (Dev) set, and the other for applying these guidelines with the Test set, resulting in annotations for 400 instances across four fallacy types (i.e., \textit{faulty generalization}, \textit{false dilemma}, \textit{fallacy of credibility}, and \textit{false causality}). We assessed the Inter-Annotator Agreement (IAA) using three different statistical measures: Cohen's Kappa, Gwet's AC1, and Krippendorff's alpha, to ensure reliability and consistency in the annotations.

% To evaluate the feasibility of our newly proposed fallacy templates, we first conduct a small trial annotation using our templates on an existing dataset of labelled fallacious arguments (i.e., LOGIC dataset~\cite{jin-etal-2022-logical}). We employ two experts in argumentation, both authors of this paper, to conduct the trial annotation on 200 instances from the LOGIC dataset spanned across 4 different fallacy types (i.e., \textit{faulty generalization}, \textit{false dilemma}, \textit{fallacy of credibility}, and \textit{false causality}). We find that our fallacy templates have a notable coverage and our annotation task has significant results on coverage and Cohen's kappa~\cite{cohen1960coefficient}. To facilitate research in fallacy instantiation, we publicly release our corpus and guidelines.~\footnote{\url{anonymous}}






% \section{Related Work}

% \paragraph{Fallacy Identification}
% \paragraph{Templates}
% ....


% Given a majority of disagreements are composed of template vs. no template, we filter out all disagreeing examples for all fallacies when conducting our experiments.% experiments in Section~\ref{sec:experiments}.

% %dataset consisting of 5 selected fallacy types. Moreover, to evaluate the feasibility of the proposed template, we use the LOGIC dataset, which encompasses 13 fallacy types, including those we have selected.


% \subsection{Template Instantiation}
% The LOGIC dataset is used, comprising 2,449 arguments. %Upon reviewing the distribution of datasets, it becomes evident that the dataset is not equally distributed, reflecting a challenge in which the statistical instances are dominated by \textit{faulty generalization} class with 18.01\%.

% We selected 250 samples across 5 fallacy types from the development set and random sampling from the training set for guideline construction and development set annotation.





% \subsection{Annotating Development Set}
% After a revised set of guidelines was created, both annotators independently annotated all 250 instances. Due to labelled instances, we annotate without identifying the fallacy type. The identification of the fallacy type is out of scope in this study. We report the results and discuss interesting findings and challenges along the way. 

%\subsection{Results and Analysis}


% During annotation, there are various instance in which annotators has uncertainty in the annotation process. So, both annotators report the confidence score for 23 instances where 18 instances are different between annotators. To improve the agreement score, we excluded uncertain instances, resulting in a slight increased in Cohen's kappa score to 0.731.

% \begin{table}[t]
%     \centering
% %    \resizebox{\columnwidth}{!}{%
%         \scriptsize
%     \begin{tabular}{p{1.8cm}|%
%     >{\raggedleft\arraybackslash}p{1cm}%
%     >{\raggedleft\arraybackslash}p{1cm}|
%     >{\raggedleft\arraybackslash}p{1cm}
%     >{\raggedleft\arraybackslash}p{1cm}}

%     \toprule
%      Fallacy Type & Template Exists (Yes/No) All ($\kappa$) & Template Exists (Yes/No) Filtered ($\kappa$) & Template Selection (1-4) All ($\kappa$) & Template Selection (1-4) Filtered ($\kappa$)\\ 
%     \midrule
%         False Dilemma & 0.634 & 0.484 & 0.501 & 0.462\\
%         Faulty Generalization & 0.276 & 0.530 & 0.383 & 0.548\\
%         False Causality & 0.790 & 0.788 & 0.740 & 0.831\\
%         Fallacy of Credibility & 0.675 & 0.760 & 0.817 & 0.944\\
%         Fallacy of Logic & 0.688 & 0.769 & 0.839 & 0.944\\
%     \midrule
%     Total & 0.730 & 0.852 & 0.645 & 0.731\\
%     \bottomrule
%     \end{tabular}
%          \caption{Agreement scores calculated across all fallacy types for 250 instances (All) and 209 instances (Filtered). We observe in the case of \textit{faulty generalization}, annotators have a low agreement unless filtering out low confident instances. Furthermore, in the case of a \textit{false dilemma}, filtering 3 instances reduces the kappa score enormously}
%     \label{tab:agreement}
% \end{table}

% We also report the Cohen's kappa between both annotators for template coverage for both all 250 instances and excluded instances. Our result is 0.730 for all instances, and 0.852 for excluded instances which indicates an excellent agreement level. Furthermore, The coverage percentage from both annotators is considerable and some fallacy types have significant improvement results namely, \textit{faulty generalization} by 0.254, \textit{fallacy of credibility} by 0.085, and \textit{fallacy of logic} by 0.081. This indicates that the templates can represent several fallacy types for the LOGIC dataset.

% \begin{table}[t]
%     \centering

% %    \resizebox{\columnwidth}{!}{%
%         \footnotesize
%     \begin{tabular}{l%
%     >{\raggedleft\arraybackslash}p{2cm}%
%     >{\raggedleft\arraybackslash}p{2.6cm}}

%     \toprule
%      Annotator & All Coverage ($\%$) & Filtered Coverage ($\%$)\\ 
%     \midrule
%         Annotator 1 & 74.8 & 76.0\\
%         Annotator 2 & 76.6 & 77.0 \\
%     \bottomrule
%     \end{tabular}
%          \caption{Coverage results for instances that can be instantiated into the template from both annotators for 250 instances (All) and 209 instances (Filtered) from LOGIC dev set.}
%     \label{tab:coverage}
% \end{table}

% \subsection{Discussion}
% \label{sec:discussion}



% \paragraph{Benefits of annotation}

% We found the benefit of annotation is the ability to explicate the implicit premise behind the fallacious argument. In Figure~\ref{fig:overview}, the other premise that we propose in our template can capture the implicit premise inside the argument to define fallacy.

% \paragraph{Potential error}

% There are multiple templates, and each template consists of several slot-fillers, all of which are in free-text form which potentially causes the error. To minimize errors during annotation, the guidelines took into account various scenarios, such as giving preference to entity slot-fillers over events, among other considerations.

% \paragraph{Implicit components}
% The annotators encountered instanced with implicit components during the annotation process. In some cases, implicitness was primarily at the level of argumentative component (i.e., claim or premise). An example of the component is as follows:

% \begin{itemize}
%     \item We should abolish the death penalty. Many respected people, such as actor, Chewbacca, have publicly stated their opposition to it.
% \end{itemize}

% On the other hand, for fallacies such as \textit{false dilemma}, sentiment and other ingredients were left implicit. This was especially the case, as annotators were instructed to think of fallacious arguments in terms of being paraphrased/rewritten as an argument from consequences argument. An example is as follows:
% \begin{itemize}
%     \item You can either support our police or Black Lives Matter.
% \end{itemize}


% OTHER SUGGESTIONS
%\title{Towards Comprehensive Fallacy Explanation:\\Introducing Templates for Detecting Fallacious Arguments}
% \title{Be Clearer! Annotating the Underlying Logic of\\Fallacious Arguments Through Templates and Slot-filling}
% From Detection to Explanation: Annotated Templates for Informal Fallacies
%In-Depth Analysis of Fallacious Arguments: Creation and evaluation of templates 
% Design and Evaluation of Templates for Deeper Analysis of Fallacious Arguments
%\title{Templates for Fallacious Arguments Towards \\Deeper Logical Error Comprehension}

% Author information can be set in various styles:
% For several authors from the same institution:
% \author{Author 1 \and ... \and Author n \\
%         Address line \\ ... \\ Address line}
% if the names do not fit well on one line use
%         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% For authors from different institutions:
% \author{Author 1 \\ Address line \\  ... \\ Address line
%         \And  ... \And
%         Author n \\ Address line \\ ... \\ Address line}
% To start a seperate ``row'' of authors use \AND, as in
% \author{Author 1 \\ Address line \\  ... \\ Address line
%         \AND
%         Author 2 \\ Address line \\ ... \\ Address line \And
%         Author 3 \\ Address line \\ ... \\ Address line}



% Templates should provide relevant information useful for identifying a fallacy. In addition, annotating fallacies poses significant challenges due to the potential for a single argument to be classified under multiple labels, underscoring the difficulty in pinpointing fallacies. 

% \newcite{reisert2018feasible} uses a template-based approach to simplify the annotation process, ensuring that it remains straightforward yet effective. We adopt this approach in order to facilitate the ease of annotation for our task.

% Referring to Template 1 as depicted in Figure~\ref{fig:dilemma}, we observe that Template 1 is chosen, with the slot filter being populated with [A] and [C]. This instantiation process, as illustrated in Figure~\ref{fig:dilemma_1}, is finalized once both (1) Premise (P), (2) Premise (P'), and Conclusion are adequately filled. We can instantiate the above example, where $A=``church''$ and $C=``good person''$. Such instantiations allow us to fulfill the desired criteria (i.e. informative, easy-to-annotate, computionally-friendly).





%herefore, the templates offer a promising approach for constructing a dataset that is both simple and concise while maintaining high quality.

% \paragraph{Easy-to-annotate } Annotating fallacies poses significant challenges due to the potential for a single argument to be classified under multiple labels, underscoring the difficulty in pinpointing fallacies. The template method proposed by ~\cite{reisert2018feasible}  uses a slot-filler approach to simplify the annotation process, ensuring that it remains straightforward yet effective. This approach is designed to facilitate ease of annotation while also being computationally efficient, meeting the criteria for being easily annotatable and computationally friendly, akin to other proposed templates in the literature.


% \paragraph{Easy-to-annotate } Annotation of fallacies is challenging, particularly given  that a fallacious argument may be assigned multiple labels, highlighting the inherent ambiguity in identifying fallacies~\cite{goffredo2022fallacious,jin-etal-2022-logical} . The template designed by~\cite{reisert2018feasible} is considered an easy, yet simple predefined template by utilizing the slot-filler approach. We desire the template by slot-filler approach for instantiating the fallacious argument to ensure ease in the annotation process. In addition, similar to XX, our proposed template has to be computationally friendly as a result of easy-to-annotate criteria. 

% \paragraph{Computationally Friendly} Similar to \newcite{reisert2018feasible}, we aim to create patterns which are not only informative and easy to annotate, but also computationally friendly.

%%% We don't do anything with CQs...
% \paragraph{Critical Questions.} The Argumentation scheme consists of various critical questions to define a strong argument or fallacious argument~\cite{walton2008informal}. Thus, the template needs to contain a structured pattern of critical questions to identify the fallacious argument. The long-term utilization of this critical question is described in \S\ref{sec::conclusion}.



%\subsection{False Dilemma Example}


% We demonstrate our template feasibility for the following example:

% \begin{figure}[t]
%     \centering\includegraphics[width=\linewidth]{figure/false_dilemma_1.jpg}
%     \caption{Instantiation of Template 1 for the False Dilemma fallacy involves the annotator receiving text input, then selecting the most suitable template from the available options. This selection process is detailed by illustrating how the slot filters are filled with specific premises and a conclusion. This example provides a clear illustration of the annotation process used to identify and categorize the False Dilemma fallacy within textual data.
% }
%     \label{fig:dilemma_1}
% \end{figure}

% \begin{itemize}
%     \item \textit{I thought you were a good person but you are not at church today (False Dilemma)}
% \end{itemize}


% Referring to Template 1 as depicted in Figure~\ref{fig:dilemma}, we observe that Template 1 is chosen, with the slot filter being populated with [A] and [C]. This instantiation process, as illustrated in Figure~\ref{fig:dilemma_1}, is finalized once both (1) Premise (P), (2) Premise (P'), and Conclusion are adequately filled. We can instantiate the above example, where $A=``church''$ and $C=``good person''$. Such instantiations allow us to fulfill the desired criteria (i.e. informative, easy-to-annotate, computionally-friendly).





% %https://github.com/irfanrob/fallacy-template
% \todo[color=yellow]{Consider merging the tables.}
% \begin{table}[t]
%     \centering
% %    \resizebox{\columnwidth}{!}{%
%         \scriptsize
%     \begin{tabular}{p{1.8cm}|%
%     >{\raggedleft\arraybackslash}p{1.2cm}%
%     >{\raggedleft\arraybackslash}p{1.2cm}
%     >{\raggedleft\arraybackslash}p{1.8cm}}

%     \toprule
%      Fallacy Type & Cohen's $\kappa$ & GWET AC1 & Krippendorff's $\alpha$\\
%     \midrule
%         \tiny{False Dilemma} & 0.501 & 0.675 & 0.498\\
%         \tiny{Faulty Generalization} & 0.383 & 0.405 & 0.385\\
%         \tiny{False Causality} & 0.740 & 0.783& 0.741\\
%         \tiny{Fallacy of Credibility} & 0.675& 0.735& 0.677\\
%         \tiny{Fallacy of Logic} & 0.688 & 0.762 & 0.688\\
%     \midrule
%     Total & 0.645& 0.664& 0.645\\
%     \bottomrule
%     \end{tabular}
%          \caption{Agreement scores for template selection in our dev set.}
%     \label{tab:dev_agreement}
% \end{table}



% \paragraph{\textbf{Dev and Train}}
% After guidelines were constructed, both expert annotators re-annotated each instance in LOGIC-DEV$_{200}$ to create our \textit{dev} set.  We then expand our annotation by annotating on top of LOGIC-TRAIN$_{200}$ to create our \textit{train} set. 
% Our agreement scores for template selection in our \textit{dev} set are shown in Table~\ref{tab:dev_agreement}. \todo[color=yellow]{What do we want to say about these results? I feel immediately the reviewer will say "Look at Hasty, Low IAA!"}

% We report the Cohen's kappa between both annotators for the template selection for all 250 instances. Even with an insignificant result for \textit{faulty generalization} type, our result is 0.645 which indicates a good agreement level.  

% , discussing results with each other and taking notes along the way. The annotation was spread into multiple rounds, and the annotator agreement (Cohen's kappa) was calculated for each round to ensure coherence and consistency were improving along the way. After all instances were annotated, annotators aggregated all notes and devised a new set of guidelines for carrying out the development stage. 

% \begin{table}[t]
%     \centering
% %    \resizebox{\columnwidth}{!}{%
%         \scriptsize
%     \begin{tabular}{p{1.8cm}|%
%     >{\raggedleft\arraybackslash}p{1.2cm}%
%     >{\raggedleft\arraybackslash}p{1.2cm}
%     >{\raggedleft\arraybackslash}p{1.8cm}}

%     \toprule
%      Fallacy Type & Cohen's $\kappa$ & GWET AC1 & Krippendorff's $\alpha$\\
%     \midrule
%         \tiny{False Dilemma} & 0.384& 0.580& 0.377\\
%         \tiny{Faulty Generalization} & 0.331& 0.386&0.332 \\
%         \tiny{False Causality} & 0.565& 0.638& 0.638\\
%         \tiny{Fallacy of Credibility} & 0.312& 0.420&0.312 \\
%         \tiny{Fallacy of Logic} & 0.403& 0.581& 0.406\\
%     \midrule
%     Total & 0.472& 0.513& 0.473\\
%     \bottomrule
%     \end{tabular}
%          \caption{Agreement scores for template selection in our train set.}
%     \label{tab:train_agreement}
% \end{table}

%\paragraph{\textbf{Train}}

%The statistics for template selection in \textit{train} are shown in Table~\ref{tab:train_agreement}. 
%We observe a drop in agreement for fallacy types such as \textit{Fallacy of Credibility} and \textit{Fallacy of Logic}, attributing to lower confidence in annotation due to more variety of structure in arguments opposed to the LOGIC-DEV$_{250}$ split.

        % \tiny{False Dilemma}  & 0.440& 0.628&0.435\\
        % \tiny{Faulty Generalization} & 0.361&0.395 &0.360\\
        % \tiny{False Causality}  & 0.652&0.710 &0.653\\
        % \tiny{Fallacy of Credibility}  & 0.492& 0.578&0.491\\
        % \tiny{Fallacy of Logic}  & 0.554& 0.682&0.557\\

        %In order to represent the aforementioned fallacy logical structure, we discuss the desired criteria for fallacy templates and our inventory of fallacy templates.


%We create our guidelines on top of LOGIC-DEV$_{200}$ via a pilot study.

% The annotation first consisted of a pilot study which was divided into multiple rounds in which agreements were calculated and disagreements were discussed amongst both annotators.   The guidelines were then discussed and updated after each subsequent round until all 200 instances in LOGIC-DEV$_{200}$ were annotated. All notes during each round were aggregated to create our final guidelines.


% \subsection{Model}

% For the model configuration, we employed LLMs, specifically the decoder-only models GPT-3.5 and GPT-4-1106-preview. The GPT model structure is based on a transformer architecture, utilizing stacked decoder-only layers to process and generate text sequentially through self-attention mechanisms and feedforward neural networks. These models were engaged using prompt engineering techniques, obviating the need for further model fine-tuning. 

% This approach mirrors real-world scenarios where acquiring a comprehensive dataset of fallacies can be challenging. We applied both zero-shot and few-shot prompting strategies in our experiments. Notably, in the context of few-shot prompting, we used one-shot and five-shot approaches. The term "shot" refers to the number of examples provided to the model within the prompt, as illustrated in \todo[color=yellow]{Figure XXX}. 

% This methodology allows us to assess the models' ability to adapt and respond accurately to fallacy detection tasks with a limited number of examples, simulating practical application conditions.


% Notably, Annotator 2 has shown greater coverage in three out of four fallacy types, especially in Fallacy of Credibility, suggesting a potential higher proficiency or a more nuanced understanding of this category. In contrast, the lower scores in Fallacy of Generalization and Fallacy of Credibility for Annotator 1 might indicate these areas as more challenging or ambiguous, possibly requiring additional clarification or training. The overall higher coverage by Annotator 2 could also imply that the templates for certain fallacies are more intuitively applicable, leading to less ambiguity in the annotation process.

% We present a comprehensive statistical analysis of the combined Few-shot-sample and Test sample. Figure~\ref{{tab:final_agreement} illustrates the distribution of fallacy instances between two annotators across five templates. This distribution suggests that we are contending with an imbalanced dataset resulting from the annotation process. For example, the Fallacy of Credibility predominantly features selections from templates 3 and 5, while False Causality most frequently appears in another specific template. This imbalance is reflective of the inherent characteristics of the LOGIC dataset. 

% Additionally, template 5 is often chosen for annotation when a fallacy instance from the LOGIC dataset does not conform to the expected definition of its fallacy type, leading to uncertainty in classification by annotators.


% \todo[color=yellow]{Add what we want to say about the overall corpus. Distribution? Template coverage? Slot-fillers? etc.}


% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{lr}
%     \toprule
%      \textbf{Fallacy Type} &\textbf{Disagree Rate} \\
%     \midrule
%         False Dilemma   & 0.32 \\
%         Faulty Generalization & 0.49 \\
%         False Causality  & 0.24 \\
%         Fallacy of Credibility  & 0.35 \\
%         % \tiny{Fallacy of Logic}  & 0.554& 0.682&0.557\\
% %    \midrule
% %    Total & 260 & 0.650 & 140 & 0.350\\
%     \bottomrule
%     \end{tabular}
%          \caption{Analysis of disagreement}
%     \label{tab:disagreement}
% \end{table}


% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{lll}
%     \toprule
%      \textbf{Fallacy Type} & \textbf{Agree} & \textbf{Disagree} \\
%     \midrule
%         False Dilemma  & 0.262 (68/260) & 0.229 (32/140) \\
%         Faulty Generalization & 0.196 (51/260) & 0.350 (49/140) \\
%         False Causality  & 0.292 (76/260)  & 0.171 (24/140) \\
%         Fallacy of Credibility  & 0.250 (65/260) & 0.250 (35/140) \\
%         % \tiny{Fallacy of Logic}  & 0.554& 0.682&0.557\\
% %    \midrule
% %    Total & 260 & 0.650 & 140 & 0.350\\
%     \bottomrule
%     \end{tabular}
%          \caption{Analysis of agreement and disagreement.}
%     \label{tab:final_agreement}
% \end{table}


% An example of all templates for \textit{false dilemma} 
 % are shown in Figure~\ref{fig:dilemma}.
 % Similar to \newcite{walton2008informal}'s argument from consequence, we adopt similar slot-fillers (i.e. $A$ and $C$), where both $A$ and $C$ our noun phrases (entity/events) explicitly mentioned in the fallacious argument. Each slot-filler in the template has an associated sentiment (\textbf{GOOD} and \textbf{BAD}), referring to the author's sentiment towards the slot-filler entity/event. \textbf{PROMOTE} and \textbf{SUPPRESS} refer to the relation between slot-fillers, where \textbf{PROMOTE} refers to trigger the consequence and \textbf{SUPPRESS} refers to preventing the consequence~\cite{hashimoto2012excitatory}. 
% including \textit{faulty generalization}, \textit{false dilemma}, \textit{false causality}, and \textit{fallacy of credibility}.




% Two templates use argument from \textit{positive} consequences while the other two templates use argument from \textit{negative} consequences, where both schemes are the form of argument from consequences scheme. 



% Using the second scheme in Figure~\ref{fig:dilemma}, we can instantiate the above example, where $A=``church''$ and $C=``good person''$. Such instantiations allow us to fulfill the desired criteria (i.e. informative, easy-to-annotate, computionally-friendly).



% Argument from Consequences has a total of three critical questions.
% However, we only adopted two critical questions since our focus is detecting fallacies rather than affirming the argument (details in \S\ref{sec:critical_questions}). 

% We proposed a new set of supporting evidence to answer the critical questions. The usage of supporting evidence is to support the premise and every template proposes a different set of supporting evidence. The pattern of the supporting evidence is created based on the logical form of each fallacy type.


% The completed dataset is divided into two parts: a few-shot example set and a test sample set, each comprising 200 instances. The few-shot example set is used to sample few-shot examples. For each fallacy class, a single template instance was randomly chosen as a one-shot example. In the context of five-shot learning, one sample from each existing template within every fallacy class was randomly selected, totaling 20 template instances. To prevent overlap between one-shot and five-shot learning samples, we manually verified the sample selection for both categories prior to experimentation. This method ensures a diverse and comprehensive dataset for evaluating the learning models' effectiveness.


% Our empirical research involved the curation of a dataset from the LOGIC dataset, comprising 500 annotated fallacious arguments across four distinct fallacy types, with each type contributing 100 arguments. The dataset was divided into a Development (Dev) set and a Training (Train) set, each consisting of 200 instances. The Train set was designated for few-shot learning examples, while the Dev set was used for testing. Furthermore, for each fallacy class, one template instance was randomly selected and used as one-shot example. For the five-shot learning approach, we randomly selected one sample from each template existing within each fallacy class, culminating in a total of four distinct templates.

% To ensure a thorough examination, the dataset was divided into three specific segments: a development (Dev) set, a Few-shot sample set, and a test set. Recognizing the challenge posed by the imbalanced class distribution across the various templates and types of fallacies, we implemented stratified sampling techniques. This approach divided the dataset into ten folds, promoting a more equitable distribution throughout. Stratified sampling was pivotal in guaranteeing that each fold accurately reflected the dataset's overall composition, preserving the proportionality of each fallacy type across the different segments.

% To mitigate the issue of imbalanced class distribution among the different fallacy types, stratified sampling was employed. This strategy facilitated an equitable allocation of the dataset into ten folds, ensuring each fallacy type was represented fairly. Consequently, the development set included 50 samples, or 10\% of the total, with each fallacy type contributing 15 samples. Similarly, the Few-shot sample set comprised 50 samples, also accounting for 10\%, with each fallacy type contributing 10 samples. The majority of the dataset, consisting of 400 samples or 80\%, was allocated to the test set. Such stratification was instrumental in ensuring that every segment of the dataset mirrored the comprehensive diversity and distribution of fallacy types, enabling a balanced and thorough evaluation.


% Figure~\ref{fig:logic} is a list of \textit{fallacy of logic} templates. The fallacy occurs when there is a logical flaw in the reasoning behind the argument, such as a propositional logic flaw. For example, ``Allowing people to possess guns is like giving a bomb to a bunch of kids.''



% In this study, we aim to evaluate the effectiveness of our newly designed fallacy templates for the purpose of explainable fallacy detection by benchmarking them against the latest advancements in state-of-the-art Large Language Models (LLMs). A central question guiding our experiment is the capability of these cutting-edge LLMs to discern the intricate structures that characterize fallacious arguments. 

% Our study addresses the challenges of fallacy detection and explanation in situations where fallacies are not predefined, reflecting the unpredictability of real-world applications. We designed experiments within zero-shot, one-shot, and five-shot learning frameworks to simulate this complexity. The experiments are intended to test the model's ability to recognize and explain fallacies under two conditions: with and without prior knowledge of the fallacy types. This methodology allows for an in-depth evaluation of the model's capability to accurately identify and articulate fallacies, mirroring the diverse conditions encountered in practical settings. Our objective is to explore the effectiveness and adaptability of LLMs in fallacy detection and explanation, contributing insights into their utility across varied real-life scenarios.


% For each target type, we sample 100 arguments randomly from LOGIC, totalling 400 arguments, where 200 arguments are taken from LOGIC's dev set (henceforth, LOGIC-DEV$_{200}$) and 200 arguments are taken from LOGIC's train set (henceforth, LOGIC-TRAIN$_{200}$). Since LOGIC's dev set does not contain certain instances of some fallacy types, we sample the missing parts from the training set.  In order to avoid duplication, we segmented LOGIC's train set before settle it into LOGIC-DEV$_{200}$ and LOGIC-TRAIN$_{200}$.


% For each target fallacy type, we sample 100 instances from LOGIC, totalling 400 instances, where 200 instances are taken from LOGIC-DEV set (henceforth, LOGIC-DEV$_{290}$) and 200 instances are taken from its train set (henceforth, LOGIC-TRAIN$_{200}$). We note that both sets preserve an equal distribution per each fallacy type.
% We note that both sets preserve an equal distribution per each fallacy type.


%, GWET AC1 (0.57), and Krippendorf's Alpha (0.54))

%We took out the coverage information for hte time being. Maybe we can have more experiment results now.
%, and obtaining a coverage score more than 74\%, indicating the feasibility of our templates. 

%shows our results. For GPT-4, an incremental context improved False Dilemma detection by 0.15 from zero to five shot. However, Faulty Generalization and Fallacy of Credibility saw a slight decrement of 0.02, indicating that more examples don't always yield better outcomes. Similarly, GPT-3.5 exhibited performance improvements in False Dilemma and False Causality with more shots, albeit Faulty Generalization dropped by 0.03 from zero to five shot. Notably, GPT-3.5 surpassed GPT-4 in False Causality by a significant margin of 0.12, although it did not outperform GPT-4 in other categories within the five-shot framework.


% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{llcccc}
% \hline
% \ xx & F$_D$ & F$_G$ & F$_C$ & F$_{credit}$ & Overall\\
% \hline
% \tiny{GPT4 zero em}  & 0.20 & 0.20 & 0.20 & 0.20 & xx\\
% \tiny{Majority}  & 0.16 & 0.06 & 0.14 & 0.09 & xx\\
% \tiny{GPT4 preview zero} & 0.05 & 0.32 & 0.24 & 0.40 & 0.25\\
% \tiny{GPT3.5 preview zero} & 0.05 & 0.30 & 0.26 & 0.14 & xx\\
% \tiny{GPT4 preview five} & 0.20 & 0.30 & 0.28 & 0.39 & 0.29 \\
% \tiny{GPT3.5 preview five} & 0.13 & 0.27 & 0.40 & 0.21 & xx \\
% \hline
% \end{tabular}
% \caption{Results of our large language model experiments. fallacy given}
% \label{LLMTemplate}
% \end{table}

%\subsection{Critical Questions}
%\label{sec:critical_questions}
%Argument from consequences consists of 3 critical questions~\cite{walton2008argumentation}, including:
%\begin{itemize}
    %\item \textbf{CQ1:} How strong is the likelihood that the cited consequences will (may, must) occur?
    %\item \textbf{CQ2:} What evidence supports the claim that the cited consequences will (may, must) occur, and is it sufficient to support the strength of the claim adequately?
    %\item \textbf{CQ3:} Are there other opposite consequences (bad as opposed to good, for example) that should be taken into account?
%\end{itemize}
%\textbf{CQ1} and \textbf{CQ2} are the critical questions that we employ in our templates.


%We discuss the construction of our dataset. 
% Our dataset consists of 400 instances, with 200 samples sourced from the LOGIC-DEV$_{200}$ set to establish annotation guidelines and another 200 samples from the LOGIC-TRAIN$_{200}$ set, utilizing these guidelines. As a result, we have allocated 200 instances for each set, henceforth designated as the 'Few-Shot-Example-Set' and the 'Test-Sample-Set,' respectively.


% We use LOGIC-DEV$_{200}$ for creation of our guidelines. Using our guidelines, we then create our \textit{dev} and \textit{train} sets using LOGIC-DEV$_{200}$ and LOGIC-TRAIN$_{200}$, respectively.

% LOGIC-DEV$_{200}$


% falalcy の logic の logic structure を formulate した、これは初めて。それをコーパスにした。

% In this work, we address logical fallacies by devising explainable fallacy templates and conducting a comprehensive evaluation using an existing fallacy dataset. We annotated 400 instances across four prevalent fallacy types, achieving substantial IAA scores. Our analysis revealed challenges in annotation consistency, particularly with instances exhibiting multiple fallacies. In experiments with Large Language Models (LLMs), the models showed difficulty in template selection despite excelling at slot filling, suggesting a promising yet complex pathway for enhancing automated fallacy detection and understanding. This work not only advances the theoretical framework for identifying logical fallacies but also underscores the practical challenges in automating such detections, paving the way for future research and development in this critical area of computational linguistics.


% In the future, we aim to conduct a large-scale annotation of a fallacy template on larger and more natural arguments.

% We plan to create a dataset for Large Language Model (LLM) experiments and expand the template selection which addresses critical questions and the challenges we encountered.

% fallacy の解析という新しいタスクを作った。可能性が広がった。
% 今回はIAAの分析にとどまっているが、本当はいろいろとできる。


% This work proposed fallacy templates as a novel tool for explaining the fallacious argument. Using the LOGIC dataset, we evaluate the templates across 4 fallacy types by conducting small trial annotation. We achieved a significant Cohen's kappa and coverage score for both all and filtered instances. 



% This study tackles logical fallacies using explainable templates, annotating 400 instances and achieving high inter-annotator agreement scores.
% Our experiments show that Large Language Models (LLMs) struggled with the fallacy logic structure identification task, highlighting future automation challenges.

